ScaMo: Exploring the Scaling Law in Autoregressive Motion Generation Model

The scaling law has been validated in various domains, such as natural language processing (NLP) and massive computer vision tasks; however, its application to motion generation remains largely unexplored. In this paper, we introduce a scalable motion generation framework that includes the motion tokenizer Motion FSQ-VAE and a text-prefix autoregressive transformer. Through comprehensive experiments, we observe the scaling behavior of this system. For the first time, we confirm the existence of scaling laws within the context of motion generation. Specifically, our results demonstrate that the normalized test loss of our prefix autoregressive models adheres to a logarithmic law in relation to compute budgets. Furthermore, we also confirm the power law between Non-Vocabulary Parameters, Vocabulary Parameters, and Data Tokens with respect to compute budgets respectively. Leveraging the scaling law, we predict the optimal transformer size, vocabulary size, and data requirements for a compute budget of $1e18$. The test loss of the system, when trained with the optimal model size, vocabulary size, and required data, aligns precisely with the predicted test loss, thereby validating the scaling law.

==> sec/3_Preliminary.tex <==
\section{Preliminary}
\subsection{Scaling law with vocabulary}
Classical scaling law only supports the fixed vocabulary, thus we follow the previous work \cite{scalingvocab} to reformulate. With the given compute budget \( C \), which is usually represented by , the goal is to get the optimal non-vocabulary model parameters \( N_{nv} \), the optimal vocabulary model parameters \( N_v \), the number of training tokens \( D \). \( N_v \) is calculated as \(N_v = Vd\), where \(V\) is the vocabulary size and d is the dimension of the model. It can be formulated as: 

\begin{equation}
\begin{aligned}
(N_v^{\text{opt}}, N_{nv}^{\text{opt}}, D^{\text{opt}}) = 
&\ \arg \min_{N_v, N_{nv}, D} \mathcal{L}(N_v, N_{nv}, D) \\ &\ \text{s.t.} \quad \text{FLOPs}(N_v, N_{nv}, D) = C,
\end{aligned}
\label{equ1}
\tag{1}
\end{equation}

According to Kaplan et al.\citep{kaplan2020scaling}, the FLOPs (\(C\)) of our Transformer-based model can be estimated as:
% \[）\]
\begin{equation}
\begin{aligned}
C \approx 6ND \approx 6(N_{nv} + Vd)D
\end{aligned}
\label{equ2}
\tag{2}
\end{equation}




\label{sec:preliminary}

==> sec/footnote.tex <==

\renewcommand{\footnoterule}{\vspace{0.5em}\hrule height 0.5pt \vspace{0.5em}

% $\dagger$
\footnote{
    Corresponding author.
}

